ModelVerification.jl: a Comprehensive Toolbox for Formally Verifying Deep Neural Networks

Deep Neural Networks (DNN) are crucial in approximating nonlinear functions across diverse applications, ranging from image classification to control. Verifying specific input-output properties can be a highly challenging task due to the lack of a single, self-contained framework that allows a complete range of verification types. To this end, we present \texttt{ModelVerification.jl (MV)}, the first comprehensive, cutting-edge toolbox that contains a suite of state-of-the-art methods for verifying different types of DNNs and safety specifications. This versatile toolbox is designed to empower developers and machine learning practitioners with robust tools for verifying and ensuring the trustworthiness of their DNN models.

==> sections/old/evaluation_old.tex <==
\section{Evaluation}\label{sec:evaluation}

This section briefly overviews how we can exploit the supported geometries to encode different input-output specifications for any particular task to be verified using \MV. For a comprehensive overview of all the toolbox functionalities, we refer the reader to the official documentation.
We divide the verification problems based on the input dimension to the neural network model to be verified.  In particular, we consider \textit{high-dimensional} problems, i.e., image-based tasks, and \textit{low-dimensional} problems, i.e., more specific control tasks based on sensors such as LiDar.

\subsection{Case study of image-based tasks.}
\subsubsection{MNIST evaluation:} The first part of this section focuses on the robustness verification of CNNs trained for classification tasks. In particular, we focus on the standard benchmark MNIST dataset \cite{MNIST}. 
%This latter comprises handwritten digits encoded as grayscale images (with a single 8-bit channel) of 28 x 28 pixels. 
The robustness verification consists of performing a series of local perturbations (i.e., local patches as shown in Fig. \ref{fig:robustness}), to find an adversarial example, e.g., a perturbated pixel (or series of pixels) close to an original training one that produces undesirable output, such as a misclassification error. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{img/robustness.pdf}
    \caption{Robustness verification using \MV.}
    \label{fig:robustness}
\end{figure}\\
In this context, \MV provides a very intuitive and straightforward way to perform the verification process. 
In detail, if we are interested in a semantic perturbation of the input image (e.g., brightness or patching perturbation), our toolbox exploits Image Convex Hull to abstract the set of all the possible perturbations and propagates this set through the CNN, performing a reachability analysis on the final output computed. An explanatory example is reported in Fig. \ref{fig:robustness}. On the other hand, if we are interested in the classic local pixel perturbation, we can exploit the geometry \textit{L-infinityBall} to encode the input perturbation and for the output the label we expect to obtain.

A key feature of our toolbox is the possibility of visualizing the reachability result of the verification process layer-by-layer. We report in Fig. \ref{fig:visualization} an explanatory example, considering a single image representing the ``five" handwritten digit and a local perturbation in the bottom left corner of the figure. In this case, \MV outputs that the CNN is robust to this specific perturbation.
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\textwidth]{img/visualization.pdf}
%     \caption{Visualization of the reachable set layer-by-layer using \MV}
%     \label{fig:visualization}
% \end{figure}\\
In the left of Fig.\ref{fig:visualization}, we report the center of the reachability set and the bounds obtained in the first layer during the propagation of the Image Convex Hull. On the right part, we report a representation of the output reachable set showing the probability distribution of each label exploiting the heatmap. As we notice, since the label ``five" has the highest value, it will be chosen by the CNN, confirming the robustness of the model.

\subsubsection{Key points detection:} In addition to the classic local robustness, \\ \MV allows to perform the verification of \textit{key points detection} task. In particular, given a CNN and a set of key points in the image, the model is robust if it can always precisely spot the location of each key point in the image, no matter the possible perturbation of the image. Hence, given a set of key points the user provides, our toolbox checks if the model is formally robust to possible different  \textit{semantic} perturbations. The originally trained networks for this specific task typically output heatmaps encoding the last layer using a softmax activation to identify the higher index corresponding to a specific label to be compared with the ground truth expected key point position. However, verifying a network based on heatmaps as output and, more specifically, with a softmax layer is complicated. 
To address this issue, $\;$\MV provides an automatic converter of this model structure into a semantically equivalent where the last layer is replaced with an \textit{average pooling} layer. Thus, the verification is transformed into a classification task. Once again we can exploit the Image Convex Hull to abstract into one geometry the set of key points in the image and to propagate this set in order to assess the robustness of the CNN. 

\subsubsection{ResNet evaluation:} we test robust trained ResNets, ResNet2b and ResNet4b. ResNet2b has two residual blocks composed of five convolutional layers plus two linear layers, while ResNet4b has four residual blocks with nine convolutional layers and two linear layers. For this evaluation, we use images from the CIFAR-10 dataset \cite{CIFAR} (composed by image size $32 \times 32$) with different occlusion perturbations. The occlusion adopted is a $6 \times 6$ black block and is randomly placed on the original image. We verified 100 images, using \textit{ImageZono} as solvers, and the results are shown in Tab. \ref{tab:results}.
\begin{table}[t]
    \centering
    \begin{tabular}{cccccc}
        \toprule
         & Holds instance & Violated instance & Unknown instance & \#Parameters & Time \\
         \midrule
         ResNet2b & 54 & 46 & 0 & 112006 & 93.51s \\
         ResNet4b & 72  & 28 & 0 & 123734 & 1086.40s \\
         \midrule
         ACAS $\phi_3$ & x & x & x& x & x\\
         ACAS $\phi_4$ &x &x &x& x & x\\
         \midrule
         FPA  & x & x & x& x & x \\
         \bottomrule
    \end{tabular}
    \caption{ResNet,ACAS and FPA verification results}
    \label{tab:results}
    \vspace{-3mm}
\end{table}




\subsection{Case study of DRL and sensor-based tasks and Neural ODE.}

In this section, we briefly describe how \MV allows even to verify different challenging DRL tasks. Our toolbox allows us to verify DRL policies easily. More specifically, due to the support of several geometric representations for the input-output specification, the encoding of the desiderata safety property is straightforward. For instance, we can encode the unsafe regions where the robot has to behave safely using convex geometries such as \textit{Hyperrectangles}. As for the encoding of the condition on the output to be verified, it is usually complicated since discrete control, for instance, requires verification that a particular action is preferred over all others simultaneously, which results in a conjunction of post conditions. To address such an issue, \MV provides an autonomous conversion of the original DNN with multiple outputs into a semantically equivalent network with only one output node that encodes the desired conjunction of postconditions, thus reducing the verification process to a single postcondition verifiable using halfspaces.
Crucially, our toolbox can verify complex safety properties in fractions of a second using a few lines of Julia code, as shown in the following listing:

\begin{minted}[frame=lines,fontsize=\tiny]{julia}
using ModelVerification as MV
# load and convert the model
onnx_path = "models/model_drl_unsafe.onnx"
model_onnx_converted = MV.convert_model(onnx_path)
model_drl = MV.build_flux_model(model)
# define the safety property
X = Hyperrectangle(low = [0.06, 0.01, 0.01, 0.01, 0.06, -1.0, 0.0], 
high = [0.7, 0.05, 0.05, 0.05, 0.7, 1.0, 1.0])
Y = Complement(HalfSpace([1.0], 0.0)) # always y > 0
# let's instantiate the Problem for the ModelVerification.jl toolbox
problem = Problem(model_drl, X, Y)
# we instantiate the 3 main components for the verification process
search_method = BFS(max_iter=200, batch_size=1)
split_method = Bisect(1)
solver = Ai2z()
# start the verification process and store the final result
result = verify(search_method, split_method, solver, problem)
\end{minted}

Moreover, \MV allows the verification of Neural ODE \cite{neuralODE} using a similar encoding provided in the listing shown above. In particular, we evaluate \MV on the Fixed Point Attractor (FPA) benchmark \cite{neuralODE}, and the results are available in Tab. \ref{tab:results}.
%Moreover, due to the vulnerability of DNNs to adversarial inputs, it is widely known that small perturbations to these sensors can result in unexpected predictions of DNNs that very likely translate into unsafe behavior. To this end, it is imperative to perform a formal verification phase before the deployment phase of these systems in the real world.
% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=0.9\textwidth]{img/eval1.pdf}
%     \caption{Robotic task. (a) represents a standard DRL benchmark simulator for mapless navigation, (b) a realistic robotic task using TurtleBot3, and (c) an explanatory example of an unsafe situation to be verified.}
%     \label{fig:robotic_verification}
% \end{figure}
% To this end, our toolbox allows us to verify DRL policies straightforwardly. To provide an intuition to the reader, suppose to consider the exemplified situation depicted in Fig. \ref{fig:robotic_verification}(c). The input space of our DNN is composed of seven continuous values that encode the lidar values and the relative position of the goal with respect to the agent's position (i.e., distance and heading). Regarding the output space, for the sake of simplicity, we consider only three discrete actions: $y_0$ that encodes a forward movement, while $y_1, y_2$ represents a left and right rotation, respectively. Suppose we want to formally verify a situation where the agent is very close to an obstacle. Hence, in this example, we are trying to encode the following situation: for every possible lidar value in the unsafe region encoded by $\mathcal{X}$, the action $y_0$ (forward movement) should always be less preferred with respect to the other two available. Formally,
% $\forall x_i \in \mathcal{X},\quad y_0 < y_1, y_2$. Hence, the formal verification process consists of finding (if it exists) an assignment in $\mathcal{X}$ such that $y_0 > y_1$ and simultaneously $y_0 > y_2$, i.e., a conjunction of two postconditions, which is often complicated to perform. 
% To address such an issue, \MV provides an autonomous conversion of the original DNN with multiple outputs into a semantically equivalent network with only one output node that encodes the desired conjunction of postconditions, thus reducing the verification process to a single postcondition verifiable using halfspaces.
% In particular, the idea is to get a result equal to $0$ only if the action $y_0$ is chosen (i.e., iff $y_0 > y_1$ and $y_0 >y_2$), and a positive output in all other cases. To this end, in this example, we add a new layer activated with $ReLU$ that computes the operation $y_1 - y_0$ and $y_2 - y_0$ in the two nodes. The only possibility of obtaining a negative value in both nodes is $y_0 > y_1$ and $y_0 >y_2$. Since these nodes are activated with $ReLU$, the final output will be $0$. On the other hand, if one between $y_1$ and $y_2$ (or both) is larger than $y_0$, we will obtain a result strictly greater than $0$, as we want.
% Hence, if the toolbox finds an assignment that produces an output equal to $0$, we have a violation point in the input safety property's domain $\mathcal{X}$. On the other hand, we have provable guarantees that the agent will never select the action corresponding to a forward movement. Crucially, our toolbox can verify complex safety properties in fractions of a second using few lines of Julia code, as shown in the following listing:

% \begin{minted}[frame=lines,fontsize=\tiny, linenos]{julia}
% using ModelVerification as MV
% # load and convert the model
% onnx_path = "models/model_drl_unsafe.onnx"
% model_onnx_converted = MV.convert_model(onnx_path)
% model_drl = MV.build_flux_model(model)
% # define the safety property
% X = Hyperrectangle(low = [0.06, 0.01, 0.01, 0.01, 0.06, -1.0, 0.0], 
% high = [0.7, 0.05, 0.05, 0.05, 0.7, 1.0, 1.0])
% Y = Complement(HalfSpace([1.0], 0.0)) # always y > 0
% # let's instantiate the Problem for the ModelVerification.jl toolbox
% problem = Problem(model_drl, X, Y)
% # we instantiate the 3 main components for the verification process
% search_method = BFS(max_iter=200, batch_size=1)
% split_method = Bisect(1)
% solver = Ai2z()
% # start the verification process and store the final result
% result = verify(search_method, split_method, solver, problem)
% \end{minted}




\subsection{Verification on Standard VNN Competition Benchmarks}
\MV also supports verifying standard benchmarks and properties evaluated in Verification of Neural Network (VNN) \cite{VNNlib,vnnComp} competition. In Tab. \ref{tab:results}, we report the result of $\alpha$-$\beta$-CROWN implemented in our toolbox employed to verify property $\phi_3$ and $\phi_4$ of ACAS xu benchmark.


==> sections/old/features_old.tex <==
\section{Toolbox Features}\label{sec:tb_features}

\MV is a toolbox developed in Julia \cite{julia} ideal for specifying algorithms in human-readable form and for the availability of useful packages for operations with convex sets such as \textit{LazySets.jl}. Our toolbox significantly extends and provides significant improvements over the existing toolbox called \texttt{NeuralVerification.jl} \cite{LiuSurvey}. In Tab. \ref{tab:improvement}, we illustrate an overview of the advancements over the previous version of the toolbox and the novel features introduced.

\subsection{\MV Novel Features}

\begin{table}[h]
    \vspace{-4mm}
    \centering
    \scriptsize
    \begin{tabularx}{\linewidth}{@{}>{\hsize=.5\hsize}X>{\hsize=1.25\hsize}X>{\hsize=1.25\hsize}X@{}}
        \toprule
        & \textbf{\texttt{NV.jl}} & \textbf{\texttt{MV.jl}} \\ 
        \midrule
        Supported\newline Layers type & 
        Linear, ReLU, Identity & 
        Linear, ReLU, Identity, Convolution, Pooling, BatchNorm, Skip connection, Parallel layer\\ 
        \midrule
        Computation graph & 
        Sequential & 
        General (such as ResNet) \\ 
        \midrule
        Hardware\newline support & 
        CPU only & 
        CPU and GPU \\ 
        \midrule
        Algorithms\newline implementations & 
        Naive - Pedagogical & 
        Efficient and Competitive \\ 
        \midrule
        Supported solvers & 
        Up to 2020 SOTA\newline (Neurify, Reluplex, etc) & 
        Up to 2023 SOTA\newline ($\alpha$-$\beta$-Crown,
        ImageStar, DeepZ, etc) \\ 
        \midrule
        Specifications & 
        Polytope (Complement)\newline No post-conditions conjunction & 
        Polytope (Complement), Image Convex Hull, post-conditions conjunction supported \\ 
          \midrule
        Verification type & 
       Standard, Robustness & 
        Standard, Robustness, Key points detection, Enumeration of (un)safe regions\\ 
        \bottomrule
    \end{tabularx}
    \caption{Comparison between \MV  and \texttt{NeuralVerification.jl}.}
    \label{tab:improvement}
    \vspace{-5mm}
\end{table}
We briefly summarize the key toolbox features below:

 \paragraph{\textbf{Support of different layer's type}:} The first big improvement with respect to the previous version of the toolbox lies in the supported layer's type. Our novel tool supports a vast range of models and verification types. In detail, \MV is designed to handle general computational graphs with versatile operators, such as ResNet \cite{ResNet}, and can be easily extended to unseen operators and novel neural network architectures. Crucially, our toolbox provides a set of model converters commonly used in the literature, such as ONNX, Tensorflow (Keras), and Pytorch, to name a few, to Flux models, a Julia library for machine learning that contains an intuitive way to define models, just like mathematical notation. In addition, Flux allows differentiable programming of cutting-edge models such as neural ODEs, typically not supported by state-of-the-art methods (e.g., $\alpha$-$\beta$-CROWN).

 \paragraph{\textbf{Efficient algorithms implementation}:} The algorithm implementations have been completely rewritten in a novel and efficient way. The code is well-structured and documented, with tutorials helpful for understanding and using the various verifiers developed. Due to its high readability structure, the user can easily either add or modify the existing solvers, support new operators, or even create custom ad hoc verification types.

 \paragraph{\textbf{Support of several geometric representations for the input-output properties}:} Specifically, a key feature of our toolbox is the support of different geometrical representations for more complex input-output specifications. In particular, for the input specification \MV supports different convex polytope geometries such as \textit{Polytope}, \textit{Hyperrectangle}, \textit{ImageConvexHull}, and \textit{ImageLinfBall}. As for the output specification, we have \textit{Polytope}, \textit{LinearSpec}. The special feature of our toolbox is that by relying on libraries that handle these geometric figures (e.g., LazySets), operations between these geometries are considerably efficient. 

 
\begin{figure}[b]
    \centering
    \includegraphics[width=0.85\textwidth]{img/reachability_results.pdf}
    \vspace{-3mm}
    \caption{Different types of verification supported in \MV}
    \label{fig:verification_types}
\end{figure}

 
\paragraph{\textbf{Different types of verification}:} In more detail, \MV allows the user to verify several types of safety properties ranging from Deep Reinforcement Learning (DRL) tasks, providing an autonomous way to verify the conjunction of post-conditions, which is typically challenging with the existing neural network verification tools, to high dimensional image-based tasks. Specifically, considering robustness verification, recent tools~\cite{VeriNet,eran,bcrown,acrown,crown} mainly focus on $L_\infty$ ball input perturbations. In contrast, we provide many different perturbation types, including \textit{Polytope} set and \textit{Image Convex Hull}, that are particularly useful for semantic perturbations or key point detection tasks that have not appeared in any previous toolbox. In addition to the reachability analysis, our toolbox provides the possibility to perform adversarial attack verification to find a single counterexample-- by exploiting one of the main methods such as Fast Gradient Sign Method (FGSM), Projected Gradient Descent (PGD) attack, and Auto-PGD. 
%\MV supports the standard robustness verification of CNNs, %as finding the maximum allowable disturbance with respect to an $\ell_p$ norm that maintains $\mathcal{F}(x)$ in the desired reachable set not only considering the classical $L_\infty$ $\epsilon$-ball, 
%but especially a wide range of different perturbation types, such as polytope set, and Image Convex Hull particularly useful for semantic perturbations. Moreover, the current version of the toolbox supports the conjunctions of postcondition, particularly useful for the verification of DRL policies. 
Finally, our toolbox includes recent approximation methods \cite{eProve} even to enumerate the set of (un)safe regions of a given safety property. We report a brief overview of the different types of verification supported in our tool in Fig. \ref{fig:verification_types}.

\paragraph{\textbf{Support of several State-of-the-art methods}:} The current version of the toolbox supports several search-reachability and optimization state-of-the-art FV methods such as $\alpha$-$\beta$-CROWN \cite{acrown,crown,bcrown}, MN-bab~\cite{ferrari2022complete}, ImageStar \cite{imageStar},  Ai2 \cite{Ai2},  ExactReach \cite{ExactReach}, and Reluplex \cite{Reluplex}.


 %Our toolbox provides a suite of state-of-the-art verification methods to provably state whether a given input-output relationship for a DNN $\mathcal{F}$ holds.
%Due to the non-linear and non-convex nature of DNNs, estimating the exact reachable set is impractical, although there are algorithms that allow us to do this, such as ExactReach \cite{} implemented in \MV. Thus, we provide a set of over-approximation-based methods to solve the verification problem either in sound or sound and complete fashion.  











\subsection{How does \MV work?}

Most existing state-of-the-art verification algorithms share a similar design logic: \textit{Branch-and-Bound} (BaB). Based on this aspect, we decided to abstract a general pipeline and modularize BaB algorithms. This results in the possibility of choosing and combining  different existing algorithms to solve the verification process optimally. In detail, all the verification algorithms implemented in our toolbox divide the hard-to-verify problem into easier problems and proceed to verify the single, easier subparts. Broadly speaking, this process can be summarized into three steps: 
\begin{enumerate}
    \item Split the input set (perturbations) into smaller sets, which we call \textit{branches}.
    \item Propagate the bounds through the model for a given branch.
    \item Check whether the bounds of the final layer satisfy the output specification.
\end{enumerate}
This process is repeated until we either find in a branch a counter-example that falsifies the property or we have verified all the branches, providing the possibility to state if the property holds formally.

The detailed workflow of \MV is depicted in \cref{fig:flow}.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\textwidth]{img/overview_mvflow.png}
    \caption{Verification process of \MV}
    \label{fig:flow}
\end{figure}\\
The user prepares an \textit{instance} to verify, which includes the model, the safety property (i.e., an input-output relationship for the model), and the desired output behavior (out-specification). In addition, the user has to indicate which solver to be employed in the verification process. As stated in the previous sections, \MV provides a vast range of state-of-the-art solvers for any type of verification (e.g., safety collision avoidance, robustness, key points detection, etc). The solver includes the desired branch split, search, and bound propagation method. 

Focusing on Fig \ref{fig:flow}, the verification process starts with the call of the \textit{verify} method, initiating all the BaB approach described before. In detail, the first sub-method that composes \textit{verify} is \textit{prepare\_problem}, which performs the preprocessing phase, such as converting the model to a computational graph, making input specification compatible with the solver, and initializing the branch bank. The \textit{search\_branches} phase is then called, which iterates through the branch bank to verify them. At each iteration, a batch of unverified branches will be extracted from the branch bank. It is worth noting that some existing formal verifiers work best exploiting GPU computation, while others heavily rely on CPU. Crucially, \MV supports both GPU and CPU-based methods. This dual support allows choosing the verifier based on the hardware conditions.

During the iteration through the branches, \textit{prepare\_method} converts and initializes the bounds of the starting node of the computational graph based on these branches. Hence, the \textit{propagate} method propagates the bounds from the start node to the end of the computational graph, finally performing \\\textit{check\_inclusion}, which states whether the bounds of the end node satisfy or not the output specification. Since we use an over-approximated reachable set, the only possibility to state the property does not hold, i.e., to find a counterexample, is to obtain a disjoint desired and computed output reachable set. If so, the verification process stops, and we can formally state the property does not hold. On the other hand, if the computed output reachable set is completely contained in the desired output set, the branch is verified, and we can continue. 

Nonetheless, the over-approximation introduced in the verification process typically prevents us from getting a firm decision in early propagations, leading to an ``unknown" answer. Hence, further problem refinement is required to get a concrete answer. In this case, the \texttt{split\_branch} method divides the current branch into smaller sub-branches and returns them to the branch bank for future verification. The process continues until either the branch bank is empty, i.e.,  all the branches are verified, or the tool finds a counterexample. \MV also allows defining a maximum computation time, i.e., a ``timeout" variable, after which the verification process stops.







==> sections/old/introduction_old.tex <==
\section{Introduction}




%the lack of a comprehensive toolbox to verify all different tasks or properties makes the use of pre-deployment verification impractical for researchers who often rely solely on empirical guarantees.

To this end, in this work, we present \MV (Fig.\;\ref{fig:overview}), the first cutting-edge toolbox that contains a suite of state-of-the-art methods for verifying different types of DNNs and safety specifications. Crucially, our toolbox allows the support of different layer types (e.g., ResNet \cite{ResNet}), currently not supported by existing state-of-the-art toolboxes \cite{NNV2.0}. Moreover, being based on Julia, ideal for specifying algorithms in human-readable form and for the availability of useful libraries for support of several geometric representations (e.g., LazySets), we support the verification of different types of input-output properties both for classification and control verification, thus providing a self-contained comprehensive toolbox. 
\vspace{-3mm}
\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{img/overview.png}
    \caption{The user provides the network, the safety property to check, and the desired solver. \MV provides an assertion of whether the safety property holds.}
    \label{fig:overview}
\end{figure}

\textit{Yet another FV toolbox?} The Formal Verification of DNNs is increasingly becoming essential for providing provable guarantees of deep learning models. We refer the interested reader to the following article for a complete taxonomy of the various state-of-the-art methods \cite{LiuSurvey}. In addition to these works, it is important to mention recent methods such as Verinet \cite{VeriNet}, MN-BaB\cite{MN-BaB}, $\alpha$-$\beta$-Crown \cite{bcrown,acrown,crown}, which provide the ability to test even complex properties, such as semantic perturbation, in addition to the classic methods focus on regression and classification tasks. However, although $\alpha$-$\beta$-Crown, for instance, was the top performer in the last three years of NN verification competition \cite{VNNComp3years}, it lacks support for different types of DNNs such as neural ODEs \cite{neuralODE}. To this end, a recent toolbox, NNV 2.0 \cite{NNV2.0}, has arisen to overcome this limitation. Still, the latter presents some limitations, such as a lack of support for different deep learning models such as ResNets \cite{ResNet}. %In contrast, our toolbox supports this and several other types of models and verification strategies, which are typically not supported by state-of-the-art solvers, making \MV the first cutting-edge self-contained tool for general verification techniques of different deep learning models.
Moreover, existing toolboxes such as Juliareach \cite{}, ReachNN \cite{}, Sherlock \cite{}, RINO \cite{}, and VenMas \cite{} mainly focus on specific verification of DNNs for Control Systems and present lack of support for different types of DNNs, as also pointed out in \cite{NNV2.0}. In contrast, our toolbox covers major state-of-the-art verifiers, including $\alpha$,$\beta$-CROWN \cite{bcrown,acrown,crown}, Image-Star \cite{imageStar}, DeepZ, Zonotope \cite{Ai2}, and different layer types as mention before, enabling the user to pick the most appropriate solver for the given problem. Hence, \MV is the first self-contained toolbox that supports different verification and safety specification types.
Our toolbox significantly extends and improves the previous version \\ \texttt{NeuralVerification.jl} and is designed to empower developers and machine learning practitioners with robust tools for verifying and ensuring the trustworthiness of their DNN models.


%The main reason to introduce a novel toolbox is that in literature, several DNN-verification methods or toolboxes \cite{NNV2.0,eran,MN-BaB} have different advantages and disadvantages based on the type of verification we want to perform, and therefore present different best-use scenario. Hence, a single self-contained toolbox for any verification type does not exist. 


%The outline of the paper is the following: in sec \ref{sec:related_work}, we briefly discuss the existing FV methods and existing toolboxes. We then proceed to present the main features of our \MV toolbox in sec \ref{sec:tb_features} and an overview of the different types of verification available using our toolbox is shown in \ref{sec:evaluation}. Finally, we conclude with the final consideration in \ref{sec:discussion}.





==> sections/related_work.tex <==
\section{Related Work}\label{sec:related_work}

The Formal Verification of DNNs is increasingly becoming essential for providing provable guarantees of deep learning models. We refer the interested reader to the following article for a complete taxonomy of the various state-of-the-art methods \cite{LiuSurvey}. In addition to these works, it is important to mention new methods such as Verinet \cite{VeriNet}, MN-BaB\cite{MN-BaB}, $\alpha$-$\beta$-CROWN \cite{bcrown,acrown,crown}, which provide the ability to test even complex properties, such as semantic perturbation, in addition to the classic methods focus on regression and classification tasks. However, although $\alpha$-$\beta$-CROWN, for instance, was the top performer in the last three years of NN verification competition \cite{VNNComp3years}, it lacks support for different types of DNNs such as neural ODEs \cite{neuralODE} or different robustness verification problems as shown above. To this end, a recent toolbox, NNV 2.0 \cite{NNV2.0}, has arisen to overcome these limitations. Still, the latter presents some limitations, such as a lack of support for different deep learning models such as ResNets \cite{ResNet}. In contrast, our toolbox supports this and several other types of models and verification strategies, which are typically not supported by state-of-the-art solvers, making \MV the first cutting-edge self-contained tool for general verification techniques of different deep learning models.
